An Origami-Inspired Design of Highly Efficient Cellular Cushion Materials

Current architectured cellular cushion materials rely mainly on damage and/or unpredictable collapse of their unit cells to absorb and dissipate energy under impact. This prevents shape recovery and produces undesirable force fluctuations that limit reusability and reduce energy absorption efficiency. Here, we propose to combine advanced manufacturing technologies with Origami principles to create a new class of architectured cellular viscoelastic cushion material which combines low weight and high energy absorption efficiency with damage resistance and full behavior customization. Each unit cell in the proposed material is inspired by the Kresling Origami topology, which absorbs impact energy by gracefully folding the different interfaces forming the cell to create axial and rotational motions. A large part of the absorbed energy is then dissipated through viscoelasticity and friction between the interfaces. The result is a nearly ideal cushion material exhibiting high energy absorbing efficiency (around 70%) combined with high energy dissipation (94% of the absorbed energy). The material is also tunable for optimal performance, reliable despite successive impact events, and achieves full shape recovery.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


